Outlier Detection as Instance Selection Method for Feature Selection in Time Series Classification

In order to allow machine learning algorithms to extract knowledge from raw data, these data must first be cleaned, transformed, and put into machine-appropriate form. These often very time-consuming phase is referred to as preprocessing. An important step in the preprocessing phase is feature selection, which aims at better performance of prediction models by reducing the amount of features of a data set. Within these datasets, instances of different events are often imbalanced, which means that certain normal events are over-represented while other rare events are very limited. Typically, these rare events are of special interest since they have more discriminative power than normal events. The aim of this work was to filter instances provided to feature selection methods for these rare instances, and thus positively influence the feature selection process. In the course of this work, we were able to show that this filtering has a positive effect on the performance of classification models and that outlier detection methods are suitable for this filtering. For some data sets, the resulting increase in performance was only a few percent, but for other datasets, we were able to achieve increases in performance of up to 16 percent. This work should lead to the improvement of the predictive models and the better interpretability of feature selection in the course of the preprocessing phase. In the spirit of open science and to increase transparency within our research field, we have made all our source code and the results of our experiments available in a publicly available repository.

==> template/title_Diplomarbeit_KF_Uni_Graz.tex <==
%%%% Time-stamp: <2013-02-02 21:30:07 vk>
%% ========================================================================
%%%% Disclaimer
%% ========================================================================
%%
%% created by
%%
%%      Karl Voit
%%


\thispagestyle{empty}  %% no page header or footer
\large  %% basic font size of the titlepage

\begin{center}
{\LARGE\bfseries\myworktitle}

\vfill

zur Erlangung des akademischen Grades eines\\[5mm]
{\LARGE\mygrade}\\[5mm]
der Studienrichtung \mystudy\\
an der \myuniversity

\vfill

über das Thema\\[10mm]

{\LARGE\bfseries\mytitle}

\vfill

eingereicht am\\
\myinstitute

Begutachter: \mysupervisor

von\\[5mm]
{\Large\bfseries\myauthor}\\[5mm]
\myhomestreet\\
\myhomepostalnumber~\myhometown

\vfill

\mysubmissiontown, \mysubmissionmonth~\mysubmissionyear

\end{center}
\normalsize %% new page, reset font size

\newpage

%% if myaddcolophon is set to "true", colophon is added:
\ifthenelse{\boolean{myaddcolophon}}{
  \newpage
  \thispagestyle{empty}  %% no page header or footer

  ~
  \vfill
  \mycolophon
}{}
\newpage

%% end of title page
%%% Local Variables:
%%% mode: latex
%%% mode: auto-fill
%%% mode: flyspell
%%% eval: (ispell-change-dictionary "de_AT")
%%% TeX-master: "../main"
%%% End:


==> template/title_Thesis_TU_Graz_-_kazemakase.tex <==
%%%% Time-stamp: <2015-04-05 11:32:08 vk>
%% ========================================================================
%%%% Disclaimer
%% ========================================================================
%%
%% created by
%%
%%      Stefan Kroboth and Karl Voit
%%
%% this title page fulfills the requirements of the corporate design
%% of Graz University of Technology (correct placement of logo)

\begin{titlepage}

%\large  %% basic font size of the titlepage

%% placing the TU Graz logo exactly as Corporate Design demands:
%%   40mm of Logo (here: 2mm margin in picture!)
%%    8mm from top and from right
%% Source: http://portal.tugraz.at/portal/page/portal/TU_Graz/Services/BDR/Oeffentlichkeitsarbeit/CD/Logo%20Anwendungsrichtlinien
\AddToShipoutPicture*{%
  \AtPageUpperLeft{%
    \hspace{\paperwidth}%
    \raisebox{-19mm}{%\baselineskip}{%
     \makebox[-4mm][r]{\includegraphics[width=42mm]{figures/TU_Graz_Logo}}
}}}%

\begin{center}
~
\vfill\vfill\vfill

\sffamily

\myauthor

\vfill

{\LARGE\bfseries\mytitle}

{\large\bfseries\mysubtitle}

\vfill\vfill\vfill\vfill

{\normalsize\bfseries\myworktitle}\\
\vfill
zur Erlangung des akademischen Grades\\
{\mygrade}\\
\vfill
eingereicht an der\\
{\normalsize\bfseries\myuniversity}

\vfill\vfill\vfill
\vfill\vfill\vfill

Betreuer\\
\mysupervisor\\
\vfill
Mitbetreuer\\
\mycosupervisor\\
%usually not mentioned on titlepage:% Evaluator: \myevaluator
\vfill
\vfill
\myinstitute\\
%Head: \myinstitutehead\\

\vfill

\myfaculty

\vfill\vfill\vfill

{\scriptsize\mysubmissiontown, \mysubmissionmonth~\mysubmissionyear}

\end{center}
\end{titlepage}

%% if myaddcolophon is set to "true", colophon is added:
\ifthenelse{\boolean{myaddcolophon}}{
  \newpage
  \thispagestyle{empty}  %% no page header or footer

  ~
  \vfill
  \mycolophon
}{}
\newpage

%% end of title page
%%% Local Variables:
%%% mode: latex
%%% mode: auto-fill
%%% mode: flyspell
%%% eval: (ispell-change-dictionary "en_US")
%%% TeX-master: "../main"
%%% End:


==> template/title_VWA.tex <==
%%%% Time-stamp: <2013-02-25 16:05:46 vk>
%% ========================================================================
%%%% Titelseite für eine Vorwissenschaftliche Arbeit
%% ========================================================================
%%
%% created by
%%
%%      Karl Voit
%%


\thispagestyle{empty}  %% no page header or footer
\large  %% basic font size of the titlepage

\begin{center}

{\LARGE\bfseries\mytitle}

\vfill

Vorwissenschaftliche Arbeit verfasst von\\[5mm]
{\Large\bfseries\myauthor}\\[5mm]
Klasse \mystudy\\[50mm]

\vfill

\includegraphics[width=3cm]{figures/institution}\\[5mm]

Betreuer: \mysupervisor

\vfill

\myinstitute\\
\myhomestreet\\
\myhomepostalnumber~\myhometown

\vfill

\mysubmissiontown, \mysubmissionmonth~\mysubmissionyear
\end{center}
\normalsize %% new page, reset font size
\newpage

%% if myaddcolophon is set to "true", colophon is added:
\ifthenelse{\boolean{myaddcolophon}}{
  \newpage
  \thispagestyle{empty}  %% no page header or footer

  ~
  \vfill
  \mycolophon
}{}
\newpage

%% end of title page
%%% Local Variables:
%%% mode: latex
%%% mode: auto-fill
%%% mode: flyspell
%%% eval: (ispell-change-dictionary "de_AT")
%%% TeX-master: "../main"
%%% End:


==> template/title_plain_maketitle.tex <==
%%%% Time-stamp: <2013-02-25 10:52:27 vk>
%% ========================================================================
%%%% Disclaimer
%% ========================================================================
%%
%% created by
%%
%%      Karl Voit
%%
%% using grml GNU/Linux, vim & LaTeX 2e

%% this is a very simple title page using LaTeX maketitle

%% if myaddcolophon is set to "true", colophon is added:
\ifthenelse{\boolean{myaddcolophon}}{
  \lowertitleback{
    \mycolophon
  }%% end lowertitleback
}{}

\title{%%
~\hfill\includegraphics[width=3cm]{figures/institution}\\[5mm] %% a logo at the upper right corner
\mytitle}

\subtitle{\mysubject}

\author{\myauthor
  \thanks{\href{http://LaTeX.TUGraz.at}{http://LaTeX.TUGraz.at}}\\
    \date{\today}
}

\maketitle


%\thispagestyle{empty}  %% no page number, header or footer



%% vim:foldmethod=expr
%% vim:fde=getline(v\:lnum)=~'^%%%%\ .\\+'?'>1'\:'='
%%% Local Variables:
%%% mode: latex
%%% mode: auto-fill
%%% mode: flyspell
%%% eval: (ispell-change-dictionary "en_US")
%%% TeX-master: "../main"
%%% End:

